Heuristics for Inequality minimization in PageRank values

PageRank is a widely used algorithm for ranking webpages and plays a significant role in determining web traffic. This study employs the Gini coefficient, a measure of income/wealth inequality, to assess the inequality in PageRank distributions and explores six deterministic methods for reducing inequality. Our findings indicate that a combination of two distinct heuristics may present an effective strategy for minimizing inequality.

==> src/fig-de-gini.tex <==
\begin{figure}[hbtp]
  \centering
  \subfigure{
    \label{fig:de-gini--mean}
    \includegraphics[width=0.98\linewidth]{out/de-gini.pdf}
  } \\[-2ex]
  \caption{Relative Gini coefficient of PageRank values (mean) obtained with three different dead-end handling strategies: \textit{teleport from dead-ends} (Teleport), \textit{self-loop dead-ends} (Loop), and \textit{self-loop all vertices} (Loop-all).}
  \label{fig:de-gini}
\end{figure}

